Accelerating Fully Homomorphic Encryption by Bridging Modular and Bit-Level Arithmetic

The dramatic increase of data breaches in modern computing platforms has emphasized that access control is not sufficient to protect sensitive user data. Recent advances in cryptography allow end-to-end processing of encrypted data without the need for decryption using Fully Homomorphic Encryption (FHE). Such computation however, is still orders of magnitude slower than direct (unencrypted) computation. Depending on the underlying cryptographic scheme, FHE schemes can work natively either at bit-level using Boolean circuits, or over integers using modular arithmetic. Operations on integers are limited to addition/subtraction and multiplication. On the other hand, bit-level arithmetic is much more comprehensive allowing more operations, such as comparison and division. While modular arithmetic can emulate bit-level computation, there is a significant cost in performance. In this work, we propose a novel method, dubbed bridging, that blends faster and restricted modular computation with slower and comprehensive bit-level computation, making them both usable within the same application and with the same cryptographic scheme instantiation. We introduce and open source C++ types representing the two distinct arithmetic modes, offering the possibility to convert from one to the other. Experimental results show that bridging modular and bit-level arithmetic computation can lead to 1-2 orders of magnitude performance improvement for tested synthetic benchmarks, as well as one real-world FHE application: a genotype imputation case study.

==> 3.3-discussion.tex <==
\subsection{Discussion on practical use of bridging}\label{ss:discussion}

In Table \ref{tab:conversion}, we present the conversion cost from \secuint\ and \secint\ to \secmod, and vice-versa, considering several bit sizes ($s \in \{4, 7, 8, 16\}$) and plaintext moduli ($t \in \{2^4+1, 2^7+1, 2^{16}+1\}$)\review{, while Table \ref{tab:general} shows the general terms}.
Converting from \secuint\ to \secmod\ does not use ciphertext multiplications; therefore it is very efficient.
A conversion from \secint\ to \secmod\ needs only two multiplications, the cost of which is amortized since expensive bit-level arithmetic multiplications are avoided.

On the other hand, conversion from \secmod\ to \secuint\ is very costly.
A ciphertext multiplication in Microsoft SEAL BFV with polynomial degree $n = 2^{15}$ takes around 0.41s using the experimental setup described in Section \ref{ss:setup}, and the smallest plaintext modulus for $n = 2^{15}$ that enables batching is $t = 2^{16}+1$.
In this scenario, a conversion from \secmod\ to \secuint\ would take more than a week, while converting from \secmod\ to \secint\ takes nearly double that time.
Practical times for the conversion could be achieved only for very small plaintext moduli, in the order of $2^4+1$. Such small moduli is meaningful only with the BGV encryption scheme, which supports much smaller plaintext moduli with batching.
Considering comparable time for ciphertext multiplication, it would be possible to convert from \secmod\ to \secuint\ under one minute for 4 bits of precision ($s = 4$ and $t = 2^4+1$), and in around 12 minutes for 7 bits of precision ($s = 7$ and $t = 2^7+1$).



==> 4.4.1-url.tex <==
\subsubsection{URL denylisting}
\label{ss:url}
\input{list/pmt_sort}

We evaluate the performance improvements provided by bridging using a URL denylisting application as a case study \cite{urldenylist}.
The application implements a Private Membership Test (PMT) protocol, a common cryptographic building block for privacy-preserving applications.
Its main operation is checking if an element is part of a database without revealing information about the element.
In this scenario, the server hosting the database is semi-trusted (honest-but-curious).

URL denylisting is the process where a URL is being checked against a known database of malicious URLs; if there is a match, the access to the website is blocked. URL denylisting can be used in conjunction with URL rewriting to protect against e-mail phishing attacks. In other words, when an email comes to the company server, its URLs are being replaced by a redirection to the service provider site, which checks whether the link is malicious or not. If it is benign, the user is automatically forwarded to the webpage. While this (supposedly) protects against phishing attacks, it introduces a huge privacy problem, since the company hosting the service can clearly see which links the users are visiting, and can potentially sell the data to other parties. 

The PMT protocol we evaluate here is composed of two main phases: setup and query. In the setup phase, the database is converted into a format that enables fast queries. The query phase is simply checking if a particular element is part of the database.
While queries are fast, the setup is expensive since it uses comparison operations. As mentioned in the previous sections, comparisons require bit-level arithmetic, leading to execution times of more than a day for databases with millions of entries. Implementing a faster setup protocol is therefore critical to the practicality of the application. 

The setup protocol is composed of three main stages: 1) The server database containing the list of malicious URLs is converted into a Bloom filter \cite{bloomfilter}. The server then informs the size of this Bloom filter $m$ to the client. 2) In the next step, the client creates a list with random permutations of \mbox{$\ceil{ {m}/({n \cdot \floor{\log_{2}{t}}} ) }$} unique integers, where $m$ is the size of the Bloom filter, $n$ is the polynomial degree, and $t$ is the plaintext modulus. The client encrypts the list with its public key and sends to the server. 3) Finally, the server runs a particular homomorphic algorithm that sorts the Bloom filter into a way only known to the client. This produces an encrypted Bloom filter in this particular order.

Out of the three stages in the setup, only the third one operates homomorphically on encrypted data. Therefore, we implemented the third stage of the setup protocol using bridging and compared its performance against the bit-level arithmetic implementation.
As shown in Fig. \ref{fig:application}, bridging provides approximately one order of magnitude of performance improvement for this application, reducing the setup time for databases with one million entries to less than three hours, instead of more than a day when bit-level arithmetic is exclusively used.

\begin{figure}[t]
	\centering
    \frame{\includegraphics[width=\linewidth]{img/application.png}}
	\caption{Execution time of the setup protocol of a URL denylisting application \cite{urldenylist} implementing the Private Membership Test.}
	\label{fig:application}
\end{figure}

This performance improvement is enabled with just a few tweaks to the sort algorithm.
Consider Listing \ref{list:pmt_sort} presenting this algorithm as an example of modifications required to enable bridged computation.
Function \texttt{sort} reorders the items of a Bloom filter in a sequence known only to the client using encrypted variable \texttt{order}. It creates a list of plaintext indices according to the protocol (lines 10-23), compares homomorphically with the encrypted list of unique permutations sent by the client (variable \texttt{order}), and composes the encrypted Bloom filter \texttt{efilter} with values in this particular order (lines 25-42).

The homomorphic operations start after line 24. There are only a few necessary changes to the algorithm: 1) In lines 1, 26, and 31 we change the return and variable types from \texttt{vector<\secuint<S>{}>} to \texttt{vector<\secmod>}, and 2) in line 35, we cast the \secbool\ type to \secmod, so the subsequent multiplication is done using modular arithmetic.
In bit-level arithmetic it is faster to cast the \texttt{vector<int>} to \secuint\ and multiply by a \secbool, since it results in a \secbool-\secuint\ multiplication instead of a \secuint-\texttt{vector<int>} multiplication. Nevertheless, with bridging it is faster to cast the \secbool\ to \secmod, instead of \texttt{vector<int>}, because \secmod-\texttt{vector<int>} multiplication is faster and less noisy than \secmod-\secmod\ multiplication.
As can be seen in Fig. \ref{fig:application}, Bridging unlocks {\it one order of magnitude} performance improvement, and it only requires minor changes to the source code.


==> list/code_log_bit.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={Logistic regression with data filtering using bit-level arithmetic.},
style=mystyle, label=list:log_bit,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <class T> vector<vector<T>>
appendCol(vector<vector<T>> m, T value)
{
  for (auto & v : m) v.push_back(value);
  return m;
}

template <int S>
vector<vector<SecureInt<S>>>
filter(vector<vector<SecureInt<S>>> m,
  SecureInt<S> threshold, vector<int> pos)
{
  for (auto & idx : pos)
  {
    for (auto & v : m)
    {
      auto cond = v[idx] > threshold;
      v[idx] = cond * threshold
            + !cond * v[idx];
    }
  }
  return m;
}

template <int S>
vector<vector<SecureInt<S>>>
mm(vector<vector<SecureInt<S>>> a,
  vector<vector<SecureInt<S>>> b)
{
  auto n = a.size();
  auto m = b.size();
  auto p = b[0].size();
  vector<vector<SecureInt<S>>> c(n);
  for (size_t i=0; i<n; i++)
  {
    for (size_t j=0; j<p; j++)
    {
      vector<SecureInt<S>> t;
      for (size_t k=0; k<m; k++)
        t.push_back(a[i][k] * b[k][j]);
      c[i].push_back(sum(t));
    }
  }
  return c;
}

template <int S>
vector<vector<SecureInt<S>>>
logreg(vector<vector<SecureInt<S>>> inputs,
  vector<vector<SecureInt<S>>> weights,
  SecureInt<S> threshold, vector<int> pos)
{
  SecureInt<S> one = _1_E;
  filter(inputs, threshold, pos);
  auto inputsU = convert(inputs, one);
  appendCol(inputsU, one);
  return mm(inputsU, weights);
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_log_bridge.tex <==
\begin{figure}[b]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={Logistic regression with data filtering using bridging.},
style=mystyle, label=list:log_bridge,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <class T> vector<vector<T>>
appendCol(vector<vector<T>> m, T value)
{
  for (auto & v : m) v.push_back(value);
  return m;
}

template <int S>
vector<vector<SecureInt<S>>>
filter(vector<vector<SecureInt<S>>> m,
  SecureInt<S> threshold, vector<int> pos)
{
  for (auto & idx : pos)
  {
    for (auto & v : m)
    {
      auto cond = v[idx] > threshold;
      v[idx] = cond * threshold
            + !cond * v[idx];
    }
  }
  return m;
}


vector<vector<SecureMod>>
mm(vector<vector<SecureMod>> a,
  vector<vector<SecureMod>> b)
{
  auto n = a.size();
  auto m = b.size();
  auto p = b[0].size();
  vector<vector<SecureMod>> c(n);
  for (size_t i=0; i<n; i++)
  {
    for (size_t j=0; j<p; j++)
    {
      vector<SecureMod> t;
      for (size_t k=0; k<m; k++)
        t.push_back(a[i][k] * b[k][j]);
      c[i].push_back(sum(t));
    }
  }
  return c;
}

template <int S>
vector<vector<SecureMod>>
logreg(vector<vector<SecureInt<S>>> inputs,
  vector<vector<SecureMod>> weights,
  SecureInt<S> threshold, vector<int> pos)
{
  SecureMod one = _1_M;
  filter(inputs, threshold, pos);
  auto inputsU = convert(inputs, one);
  appendCol(inputsU, one);
  return mm(inputsU, weights);
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_max_bit.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={Bit-level depth-optimized max function.},
style=mystyle, label=list:max_bit,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]









template <int S> vector<SecureInt<S>>
indices(vector<SecureInt<S>> v)
{
  int size = v.size();
  vector<SecureInt<S>> idx;
  vector<vector<SecureInt<S>>> m(size);
  for (int i=0; i < size; i++)
  {
    for (int j=i+1; j < size; j++)
    {
      auto cond = v[i] > v[j];
      m[i].push_back(SecureInt<S>(cond));
      m[j].push_back(SecureInt<S>(!cond));
    }
    idx.push_back(product(m[i]));
  }
  return idx;
}

template <int S> SecureInt<S>
select(vector<SecureInt<S>> idx,
  vector<SecureInt<S>> v)
{
  int size = v.size();
  vector<SecureInt<S>> r;
  for (int i=0; i < size; i++)
    r.push_back(idx[i] * v[i]);
  return sum(r);
}

template <int S> SecureInt<S>
max(vector<SecureInt<S>> v)
{
  return select(indices(v), v);
}

\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_max_bridge.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={Depth optimized max function with bridging.},
style=mystyle, label=list:max_bridge,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <class T> vector<SecureMod>
convert(vector<T> v)
{
    vector<SecureMod> u;
    for (auto & e : v)
        u.push_back(SecureMod(e));
    return u;
}

template <int S> vector<SecureMod>
indices(vector<SecureInt<S>> v)
{
  int size = v.size();
  vector<SecureMod> idx;
  vector<vector<SecureMod>> m(size);
  for (int i=0; i < size; i++)
  {
    for (int j=i+1; j < size; j++)
    {
      auto cond = v[i] > v[j];
      m[i].push_back(SecureMod(cond));
      m[j].push_back(SecureMod(!cond));
    }
    idx.push_back(product(m[i]));
  }
  return idx;
}

SecureMod
select(vector<SecureMod> idx,
    vector<SecureMod> v)
{
  int size = v.size();
  vector<SecureMod> r;
  for (int i=0; i < size; i++)
    r.push_back(idx[i] * v[i]);
  return sum(r);
}

template <int S> SecureMod
max(vector<SecureInt<S>> v)
{
  return select(indices(v), convert(v));
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_mux_bit.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={The multiplexer function using bit-level arithmetic.},
style=mystyle, label=list:mux_bit,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <int S> SecureInt<S>
mux(SecureInt<S> input, SecureInt<S> item,
    SecureInt<S> t, SecureInt<S> f)
{
    auto cond = input == item;
    return cond * t
        + !cond * f;
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_mux_bridge.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={The multiplexer function with bridging.},
style=mystyle, label=list:mux_bridge,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <int S> SecureMod
mux(SecureInt<S> input, SecureInt<S> item,
    SecureInt<S> t, SecureInt<S> f)
{
    auto cond = input == item;
    return cond * SecureMod(t)
        + !cond * SecureMod(f);
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_pks_bit.tex <==
\begin{figure}[h]

%\scriptsize
% \vbox to 600pt {
\noindent\begin{minipage}{.50\textwidth}
\begin{lstlisting}[language=C++,
caption={Private Keyword Search using bit-level arithmetic.},
style=mystyle, label=list:pks_bit,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <int S> SecureInt<S>
pks(vector<SecureInt<S>> v, SecureInt<S> k)
{
    vector<SecureInt<S>> r;
    for (size_t i=0; i < v.size(); i++)
    {
        auto eq = i == k;
        auto sel = eq * v[i];
        r.push_back(sel);
    }
    return sum(r);
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}


% }
\end{figure}


==> list/code_pks_bridge.tex <==
\begin{figure}[h]
%\scriptsize
\noindent\begin{minipage}{.50\textwidth}
\begin{lstlisting}[language=C++,
caption={Private Keyword Search with bridging.},
style=mystyle, label=list:pks_bridge,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <int S> SecureMod
pks(vector<SecureInt<S>> v, SecureInt<S> k)
{
    vector<SecureMod> r;
    for (size_t i=0; i < v.size(); i++)
    {
        auto eq = i == k;
        auto sel = eq * SecureMod(v[i]);
        r.push_back(sel);
    }
    return sum(r);
}
\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


% \begin{figure}[t]
% %\scriptsize
% \noindent\begin{minipage}{.45\textwidth}
% \begin{lstlisting}[language=C++,
% caption={Private Keyword Search with bridging.},
% style=mystyle, label=list:pks_bit,
% %framexrightmargin=-37pt,
% % xleftmargin=0.4cm,
% % xrightmargin=-0.12\linewidth,
% % linewidth=0.88\linewidth
% ]
% template <int S> SecureMod
% pks(vector<SecureInt<S>> v, SecureInt<S> k)
% {
%     vector<SecureMod> r;
%     for (size_t i=0; i < v.size(); i++)
%     {
%         auto eq = i == k;
%         auto sel = eq * SecureMod(v[i]);
%         r.push_back(sel);
%     }
%     return sum(r);
% }
% \end{lstlisting}
% \end{minipage}
% % \vspace{\lstbspace}
% \end{figure}


==> list/code_sort_bit.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={Depth-optimized sorting algorithm using bit-level arithmetic.},
style=mystyle, label=list:sor_bit,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]









template <int S> vector<SecureInt<S>>
indices(vector<SecureInt<S>> v)
{
  int size = v.size();
  vector<SecureInt<S>> idx;
  vector<vector<SecureInt<S>>> m(size);
  for (int i=0; i < size; i++)
  {
    for (int j=i+1; j < size; j++)
    {
      auto cond = v[i] > v[j];
      m[i].push_back(SecureInt<S>(cond));
      m[j].push_back(SecureInt<S>(!cond));
    }
    idx.push_back(sum(m[i]));
  }
  return idx;
}

template <int S> vector<SecureInt<S>>
select(vector<SecureInt<S>> idx,
  vector<SecureInt<S>> v)
{
  int size = v.size();
  vector<SecureInt<S>> r;
  for (int i=0; i < size; i++)
  {
    vector<SecureInt<S>> t;
    for (int j=0; j < size; j++ )
      t.push_back((i == idx[j]) * v[j]);
    r.push_back(sum(t));
  }
  return r;
}

template <int S> vector<SecureInt<S>>
sort(vector<SecureInt<S>> v)
{
  return select(indices(v), v);
}

\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/code_sort_bridge.tex <==
\begin{figure}[t]
%\scriptsize
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++,
caption={Depth-optimized sorting algorithm using bridging.},
style=mystyle, label=list:sor_bridge,
%framexrightmargin=-37pt,
% xleftmargin=0.4cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <class T> vector<SecureMod>
convert(vector<T> v)
{
    vector<SecureMod> u;
    for (auto & e : v)
        u.push_back(SecureMod(e));
    return u;
}

template <int S> vector<SecureInt<S>>
indices(vector<SecureInt<S>> v)
{
  int size = v.size();
  vector<SecureInt<S>> idx;
  vector<vector<SecureInt<S>>> m(size);
  for (int i=0; i < size; i++)
  {
    for (int j=i+1; j < size; j++)
    {
      auto cond = v[i] > v[j];
      m[i].push_back(SecureInt<S>(cond));
      m[j].push_back(SecureInt<S>(!cond));
    }
    idx.push_back(sum(m[i]));
  }
  return idx;
}

template <int S> vector<SecureMod>
select(vector<SecureInt<S>> idx,
  vector<SecureMod> v)
{
  int size = v.size();
  vector<SecureMod> r;
  for (int i=0; i < size; i++)
  {
    vector<SecureMod> t;
    for (int j=0; j < size; j++ )
      t.push_back((i == idx[j]) * v[j]);
    r.push_back(sum(t));
  }
  return r;
}

template <int S> vector<SecureMod>
sort(vector<SecureInt<S>> & v)
{
  return select(indices(v), convert(v));
}


\end{lstlisting}
\end{minipage}
% \vspace{\lstbspace}
\end{figure}


==> list/pmt_sort.tex <==
\begin{figure}[h!]
% \vspace{-0.2 cm}
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=C++, caption={
Relevant function of the setup protocol of the URL denylisting application with bridging.
},
style=mystyle, 
label=list:pmt_sort,
xleftmargin=0.45cm,
% xrightmargin=-0.12\linewidth,
% linewidth=0.88\linewidth
]
template <int S> vector<SecureMod>
sort (int logt, vector<int> filter,
  const vector<SecureUint<S>> & order)
{
  using SecUint = SecureUint<S>;
  auto s = order.size();
  auto n = SecureMod::slots();
  auto nsp = n*s*logt;
  filter.resize(nsp, 0);
  vector<vector<unsigned>> f;
  for (int i=0; i<s; i++)
  {
    vector<unsigned> poly;
    for (int j=0; j<n; j++)
    {
      unsigned plain = 0;
      for (int k=0; k<logt; k++)
        plain = (plain<<1) +
          bool( filter[i+(j*logt+k)*s] );
      poly.push_back(plain);
    }
    f.push_back(poly);
  }
  
  $//$vector<SecUint> efilter;
  vector<SecureMod> efilter;
  for ( int i=0; i<s; i++ )
  {
    const auto & c = order[i];
    $//$vector<SecUint> partial_res;
    vector<SecureMod> partial_res;
    for (int j=0; j<s; j++)
    {
      $//$auto tmp = (c==j) * SecUint(f[j]);
      auto tmp = SecureMod(c==j) * f[j];
      partial_res.push_back(tmp);
    }
    $//$ low depth array summation  
    auto r = sum(partial_res);
    efilter.push_back(r);
  }
  return efilter;
}
\end{lstlisting}
\end{minipage}
\vspace{-0.6 cm}
% \vspace{-0.1 cm}
\end{figure}

==> table/table_generalization.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
         \review{\secuint{}}                & \review{mul}   & \review{\normalfont{0}}                                                           \\
         \review{\normalfont{to}}           & \review{add}   & \review{\normalfont{$2 \cdot (s - 1)$}}                                           \\
         \review{\secmod{}}                 & \review{depth} & \review{\normalfont{0}}                                                           \\ \hline
         \review{\secint{}}                 & \review{mul}   & \review{\normalfont{2}}                                                           \\
         \review{\normalfont{to}}           & \review{add}   & \review{\normalfont{$2s + 1$}}                                                    \\
         \review{\secmod{}}                 & \review{depth} & \review{\normalfont{1}}                                                           \\ \hline
         \review{\secmod{} \normalfont{to}} & \review{mul}   & \review{\tiny{$t \cdot (s + \floor{\log_2{(t-1)}} + \omega(t-1) - 1)$}}           \\
         \review{\secuint{}}                & \review{depth} & \review{\scriptsize{$\ceil{\log_2{(t-1)}} + 1$}}                                  \\ \hline
         \review{\secmod{} \normalfont{to}} & \review{mul}   & \review{\tiny{$2 \cdot t \cdot (s + \floor{\log_2{(t-1)}} + \omega(t-1) - 1)+2$}} \\
         \review{\secint{}}                 & \review{depth} & \review{\scriptsize{$\ceil{\log_2{(t-1)}} + 2$}}                                  \\
    \end{tabular}
    \caption{\review{General terms for the number of multiplications (mul), number of additions (add), and multiplicative depth (depth) for converting from \secuint\ and \secint\ to \secmod\ and vice-versa, where $s$ is the number of encrypted bits in the \secuint/\secint\ variable, $t$ is the plaintext modulus, and $\omega(\cdot)$ is the Hamming weight.}}
    \label{tab:general}
\end{table}

==> table/table_sec3-3.tex <==
\begin{table*}[!th]
\centering
\begin{tabular}{cc|ccc|ccc|cc|cc}
  &   & \multicolumn{3}{c|}{\secuint\ \texttt{to} } & \multicolumn{3}{c|}{\secint\ \texttt{to} } & \multicolumn{2}{c|}{\secmod\ \texttt{to} } & \multicolumn{2}{l}{\secmod\ \texttt{to} } \\ 
  \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\secmod{}}        & \multicolumn{3}{c|}{\secmod{}}      & \multicolumn{2}{c|}{\secuint{}}     & \multicolumn{2}{c}{\secint{}}     \\ \hline
s  & t & mul     & add     & depth    & mul     & add    & depth    & mul            & depth         & mul           & depth        \\ \hline
\normalfont{4}  & \unboldmath \( 2^{4} +1 \)  & \normalfont{0}         & \normalfont{6}         & \normalfont{0}       & \normalfont{2}         & \normalfont{9}        & \normalfont{1}       & \normalfont{136}              & \normalfont{5}            & \normalfont{274}             & \normalfont{6}           \\ \hline
\normalfont{7}  & \unboldmath \( 2^{7} +1 \)  & \normalfont{0}         & \normalfont{12}        & \normalfont{0}       & \normalfont{2}         & \normalfont{15}       & \normalfont{1}       & \normalfont{1778}             & \normalfont{8}            & \normalfont{3558}            & \normalfont{9}           \\ \hline
\normalfont{8}  & \unboldmath \( 2^{16} +1 \)  & \normalfont{0}         & \normalfont{14}        & \normalfont{0}       & \normalfont{2}         & \normalfont{17}       & \normalfont{1}       & \normalfont{1572888}          & \normalfont{17}           & \normalfont{3145778}         & \normalfont{18}          \\ \hline
\normalfont{16} & \unboldmath \( 2^{16} +1 \)  & \normalfont{0}         & \normalfont{30}        & \normalfont{0}       & \normalfont{2}         & \normalfont{33}       & \normalfont{1}       & \normalfont{2097184}          & \normalfont{17}           & \normalfont{4194370}         & \normalfont{18}         \\
\end{tabular}
\caption{Number of ciphertext additions and multiplications, and multiplicative depth for converting from \secuint\ and \secint\ to \secmod, and vice-versa. The results show that \secmod{} to \secuint\ and \secint\ conversion is impractical. The overhead from ciphertext additions for converting from \secmod\ to \secuint\ and \secint\ is negligible and not included.}
\label{tab:conversion}
\end{table*}



